On the Theorem of the Three Perpendiculars

We show that the theorem of the three perpendiculars holds in any n-dimensional space form.

==> Macros.tex <==

\newcommand{\nc}{\newcommand}
\newcommand{\df}{\def}
\RequirePackage{ifthen}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%racourciss divers
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\df\ie#1{{\it \mbox{i.\hspace{0.06em}e.\ifthenelse{\equal{#1}{,}}{\hspace{0.06em},}{\ #1}}}}
\df\eg#1{{\it \mbox{e.\hspace{0.06em}g.\ifthenelse{\equal{#1}{,}}{\hspace{0.06em},}{\ #1}}}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Citations dans Theorem
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\nc{\cit}[2][]{\ifthenelse{\equal{#1}{}}{\rm \cite{#2}}{\rm \cite[#1]{#2}}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Gestions des {|}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 
% usage:
% \set(:bla ... | blajjxo..:) (in display)
% \set[2](: | :) (if nested sets, gives the nesting degree, up to 4)
% \seti(: | :)  or \seti[2](: | :) (outside display (i=inline))


\makeatletter
\newlength{\JR@setLa}
\newlength{\JR@setLb}
\newlength{\JR@setLc}
\newlength{\JR@setLd}
\newlength{\JR@setLe}
\nc{\JR@setMta}{}
\nc{\JR@setMtb}{}
\nc{\JR@setMtc}{}
\nc{\JR@setMtd}{}

\nc{\JR@setMt}[1]{
\ifthenelse{#1=1}{\JR@setMta}{}
\ifthenelse{#1=2}{\JR@setMtb}{}
\ifthenelse{#1=3}{\JR@setMtc}{}
\ifthenelse{#1=4}{\JR@setMtd}{}
}


\nc{\JR@max}[3]{\ifthenelse{\lengthtest{\the#1>\the#2}}
           {\setlength{#3}{#1}}
           {\setlength{#3}{#2}}}


\nc{\JR@setds}{}
\nc{\JR@setSD}[4][]{
 \ifthenelse{\equal{#1}{}}
   {\renewcommand{\JR@setds}{}}
   {\renewcommand{\JR@setds}{\displaystyle}}
 \settoheight{\JR@setLa}{\ensuremath{\JR@setds{#2}}}
 \settoheight{\JR@setLb}{\ensuremath{\JR@setds{#3}}}
 \settodepth{\JR@setLc}{\ensuremath{\JR@setds{#2}}}
 \settodepth{\JR@setLd}{\ensuremath{\JR@setds{#3}}}
 \settowidth{\JR@setLe}{\ensuremath{\JR@setds{\left.\right.}}}
 \JR@max{\JR@setLc}{\JR@setLd}{\JR@setLc}
 \JR@max{\JR@setLa}{\JR@setLb}{\JR@setLa}
 \addtolength{\JR@setLa}{\JR@setLc}
 \ifthenelse{#4=1}{\renewcommand{\JR@setMta}{\rule[-\JR@setLc]{0pt}{\JR@setLa}}}{}
 \ifthenelse{#4=2}{\renewcommand{\JR@setMtb}{\rule[-\JR@setLc]{0pt}{\JR@setLa}}}{}
 \ifthenelse{#4=3}{\renewcommand{\JR@setMtc}{\rule[-\JR@setLc]{0pt}{\JR@setLa}}}{}
 \ifthenelse{#4=4}{\renewcommand{\JR@setMtd}{\rule[-\JR@setLc]{0pt}{\JR@setLa}}}{}
} 
 

\df\SetEx[#1,#2](:#3|#4:){
 \JR@setSD[#2]{#3}{#4}{#1}
 \left\{\JR@setMt{#1} #3\right.\left|\rule{.9\JR@setLe}{0pt}#4 \JR@setMt{#1}\right\}
}


\nc{\set}[1][1]{\SetEx[#1,ds]}
\nc{\seti}[1][1]{\SetEx[#1,]}



\makeatother


